Deep Manifold Transformation for Nonlinear Dimensionality Reduction

Manifold learning-based encoders have been playing important roles in nonlinear dimensionality reduction (NLDR) for data exploration. However, existing methods can often fail to preserve geometric, topological and/or distributional structures of data. In this paper, we propose a deep manifold learning framework, called deep manifold transformation (DMT) for unsupervised NLDR and embedding learning. DMT enhances deep neural networks by using cross-layer local geometry-preserving (LGP) constraints. The LGP constraints constitute the loss for deep manifold learning and serve as geometric regularizers for NLDR network training. Extensive experiments on synthetic and real-world data demonstrate that DMT networks outperform existing leading manifold-based NLDR methods in terms of preserving the structures of data.

==> Main_hyper-paras.tex <==
\begin{table}[h]
  \footnotesize
  \centering
  \caption{Dataset-dependent Hyperparameters for DMT networks}
  \begin{tabular}{@{}cccc@{}}
  \toprule
  Dataset         & Network Structure                 & $Q$  & Batchsize \\ \midrule
  Swiss Roll      & [-1, 1000, 900, 800, 700, 500, 2] & 10   & 800       \\
  S-Curve         & [-1, 1000, 900, 800, 700, 500, 2] & 10   & 800       \\
  Servered Sphere & [-1, 1000, 900, 800, 700, 500, 2] & 10   & 800       \\
  SpheresA        & [-1, 1000, 900, 800, 700, 500, 2] & 10   & 10000     \\
  SpheresB        & [-1, 1000, 900, 800, 700, 500, 2] & 10   & 5500      \\
  Coil20          & [-1, 1000, 900, 800, 700, 500, 2] & 10   & 1440      \\
  Coil100         & [-1, 1000, 900, 800, 700, 500, 2] & 10   & 2400      \\
  MNIST           & [-1, 1000, 900, 800, 700, 500, 2] & 15   & 4000      \\ 
  Fashion-MNIST   & [-1, 1000, 900, 800, 700, 500, 2] & 10   & 4000      \\ 
  \bottomrule
  \end{tabular}
  \label{tbl:Main_hyper-paras}
  \end{table}
